ODEFormer: Symbolic Regression of Dynamical Systems with Transformers

We introduce ODEFormer, the first transformer able to infer multidimensional ordinary differential equation (ODE) systems in symbolic form from the observation of a single solution trajectory. We perform extensive evaluations on two datasets: (i) the existing "Strogatz" dataset featuring two-dimensional systems; (ii) ODEBench, a collection of one- to four-dimensional systems that we carefully curated from the literature to provide a more holistic benchmark. ODEFormer consistently outperforms existing methods while displaying substantially improved robustness to noisy and irregularly sampled observations, as well as faster inference. We release our code, model and benchmark dataset publicly.

==> main_text.tex <==
\section{Introduction}\label{sec:intro}

% PREVIOUS TEXT (included in the following three paragraphs)
% The recent triumphs of machine learning (ML)  offer plenty of enthusiasm for accelerating scientific discovery~\citep{davies2021advancing, degrave2022magnetic, jumper2021highly}. Yet, this progress mostly stems from deep learning, which involves large, overparameterized models which typically operate as black-boxes, void of any interpretability. Symbolic regression (SR) consists in predicting an explicit mathematical expression from the data, and hence appears as a promising alternative to infer natural laws in an interpretable fashion, and has already been used to accelerate scientific discoveries~\citep{Archiga2021AcceleratingUO,Udrescu2021SymbolicPD,butter2021back}. 

% Symbolic regression is most commonly used to infer a function $g$ from a set of observations $(x,g(x))$. However, in many fields of science, understanding a system involves deciphering its dynamics, i.e., inferring the function $f$ governing its evolution via $\dot x = f(x)$. This task, often called system identification, amounts to inferring a set of differential equations $f$ from the observation of trajectories, $(t, x(t,s))$, for initial conditions $s$. One could in principle consider the second setting as a subset of the first, since it consists in performing symbolic regression on the derivatives $\dot x$ instead of $x$ directly. But in practive, computing the derivative $\dot x$ must be performed via finite differences, which can become intractably noisy in presence of noise or irregularly sampled data, particularly as the dimensionality increases. 

% On a more fundamental level, even assuming that we have access to noiseless derivatives, symbolic regression of dynamical systems remains challenging in two regards: (i) the data points are not independent, since they come from the same trajectory, and (ii) qualitative patterns are much harder to identify. For example, while low-degree polynomials are usually easy to recognize qualitatively, they become much harder to identify inside an ODE, as they can give rise to all sorts of complex behaviors such as oscillations and chaos. For all these reasons, building methods specifically designed to model dynamical systems is both a difficult and important problem to address.

% NEW TEXT
%\subsection{Motivation}



Recent triumphs of machine learning (ML) spark growing enthusiasm for accelerating scientific discovery~\citep{davies2021advancing, jumper2021highly,degrave2022magnetic}.
In particular, inferring dynamical laws governing observational data is an extremely challenging task that is anticipated to benefit substantially from modern ML methods.
Modeling dynamical systems for forecasting, control, and system identification has been studied by various communities within ML.
Successful modern approaches are primarily based on advances in deep learning, such as neural ordinary differential equation (NODE) (see \citet{chen2018neural} and many extensions thereof).
However, these models typically lack interpretability due to their black-box nature, which has inspired extensive research on explainable ML of overparameterized models \citep{tjoa2020survey,dwivedi2023explainable}.
An alternative approach is to directly infer human-readable representations of dynamical laws.
% However, these models typically lack interpretability due to their black-box nature, which impede scientific insights.
% While the interpretability of highly overparameterized models has been brought into the focus of the community, there is still a substantial gap in analytical, directly human-readable representations of dynamical laws.

This is the main goal of symbolic regression (SR) techniques, which make predictions in the form of explicit symbolic mathematical expressions directly from observations.
Recent advances in SR make it a promising alternative to infer natural laws from data and have catalyzed initial successes in accelerating scientific discoveries~\citep{Archiga2021AcceleratingUO,Udrescu2021SymbolicPD,butter2021back}.
So far, SR has most commonly been used to infer a function $g(x)$ from paired observations $(x, g(x))$ -- we call this \emph{functional SR}.
However, in many fields of science, understanding a system involves deciphering its dynamics, i.e., inferring a function $f(x)$ governing its evolution via an ODE $\dot{x} = f(x)$ -- we call this setting \emph{dynamical SR}.
The task is then to uncover $f$ from an observed solution trajectory $(t, x(t))$, where observations of $x(t)$ may be noisy and times $t$ may be irregularly sampled.

%In principle, dynamical SR, inferring $f$ from $(t, x(t))$, can be framed as functional SR for $(x(t), \dot{x}(t))$ pairs.
%However, this approach implies the computation of numerical approximations of $\dot{x}(t)$ from observations (typically via finite differencing), a severe challenge for noisy and irregularly sampled data as highlighted by~\citet{becker2023predicting} and confirmed by our results, in particular for higher-dimensional systems.
%; (iii) while it is reasonable to assume that measurements of time $t$ are essentially noiseless in modern lab settings, the system measurements $x(t)$ are typically noisy. Hence, functional SR on $(x(t), \dot{x}(t))$ has to deal with both noisy inputs of the target function and noisy outputs, where furthermore the noises on input and output observations are not independent.
%Hence, scalable and efficient methods specifically tailored to dynamical SR are an important and difficult problem to address.

\begin{figure}[t]
    \centering
    \vspace{-6mm}
    \begin{subfigure}[b]{.24\linewidth}
    \includegraphics[width=\linewidth]{figs/odebench/odebench_9.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{.24\linewidth}
    \includegraphics[width=\linewidth]{figs/odebench/odebench_16.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{.24\linewidth}
    \includegraphics[width=\linewidth]{figs/odebench/odebench_27.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{.24\linewidth}
    \includegraphics[width=\linewidth]{figs/odebench/odebench_40.pdf}
    \end{subfigure}\\[-5mm]
    \begin{subfigure}[b]{.24\linewidth}
    \includegraphics[width=\linewidth]{figs/odebench/odebench_52.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{.24\linewidth}
    \includegraphics[width=\linewidth]{figs/odebench/odebench_54.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{.24\linewidth}
    \includegraphics[width=\linewidth]{figs/odebench/odebench_62.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{.24\linewidth}
    \includegraphics[width=\linewidth]{figs/odebench/odebench_63.pdf}
    \end{subfigure}
    \vspace{-3mm}

    \caption{\textbf{\odeformer{} reconstructs noisy and irregularly sampled trajectories well.} Ground truth trajectories (thick lines) are corrupted (5\% noise) and unevenly sampled (50\% of the equally spaced points are dropped uniformly at random), yielding the observed trajectories (dots) from which \odeformer{} infers a symbolic ODE. %We then integrate this ODE from the original initial condition for the prediction (thin lines). 
    Integrating this ODE from the original initial condition (thin lines) shows that it approximates the observations well.
    We display 1, 2, 3 and 4 dimensional ODEs from our dataset \odebench{} -- see \cref{app:odebench} for details and results on the remaining ODEs. %\odeformer{} is robust to noise and uneven samples, but struggles for complex chaotic systems such as the Lorenz attractor, especially for long time horizons (indeed, chaotic solutions are statistically rare in the training data).
    }\label{fig:examples}
    \vspace{-4mm}
\end{figure}


\xhdr{Contributions.}
In this work, we introduce \odeformer{}, the first Transformer trained to infer dynamical laws in the form of multidimensional ODEs from observational (noisy, irregularly sampled) data.
It relies on large-scale training of a sequence-to-sequence transformer on diverse synthetic data, leading to efficient and scalable inference for unseen trajectories. %-- unlike most existing approaches, it does not require separate training for each new system.

Faced with the lack of benchmarks for dynamical SR (the only existing one, called ``Strogatz dataset'' \citep{la2021contemporary}, contains only seven two-dimensional systems, and is not integrated with sufficient precision \citep{omejc2023probabilistic}), we also introduce \odebench{}, a more extensive dataset of 63 ODEs curated from the literature, which model real-world phenomena in dimensions one to four (see \cref{app:odebench} for details).
%. 
On both benchmarks, \odeformer{} achieves higher accuracy than existing methods for irregular, noisy observations while being faster than most competitors.
Our code, models and benchmark dataset are available publicly at
\texttt{anonymized}.
% , and incorrectly annotated (contrary to its description it in fact contains no chaotic systems).
% Proper evaluation of dynamical SR being notoriously elusive \citep{la2021contemporary,matsubara2022rethinking}, we take particular care in our empirical evaluation and measure in- and certain out-of-distribution generalization.
% The primary existing benchmark dataset, called ``Strogatz dataset'' \citep{la2021contemporary}, is small (7 ODEs), non-diverse (only two-dimensional ODEs), and not integrated with sufficient precision \citep{omejc2023probabilistic}.
% , making symbolic recovery almost impossible for existing methods 
% While we still evaluate our model on this existing benchmark,% We also provide carefully integrated solution trajectories for different initial conditions.


\xhdr{Problem setting and overview.}
We assume observations $\{(t_i, x_i)\}_{i \in [N]}$,\footnote{We use the notation $[N] := \{1, \ldots, N\}$ and $\dot{x}$ for the temporal derivative.} of a solution $x(t)$ of
\begin{equation*}
    \dot{x} = f(x), \quad \text{for some } f: \R^{\din} \to \R^{\din}\:,
\end{equation*}
where $x_i$ can be noisy observations of $x(t_i)$ with irregularly sampled $t_i$.
The task is to infer $f$ in symbolic form from the data $\{(t_i, x_i)\}_{i \in [N]}$.
% We note that this includes higher-order as well as non-autonomous ODE systems, because every $d$-dimensional, $k$-th order ODE can be written equivalently as a $(k\cdot d)$-dimensional first order ODE and every non-autonomous $d$-dimensional first order ODE can be written equivalently as a $(d+1)$-dimensional autonomous first order ODE \citep{smale1974differential}.
As illustrated in \cref{fig:sketch}, \odeformer{} is based on large-scale pre-training on ``labelled'' examples that consist of randomly generated symbolic mathematical expressions as the prediction target $f$ and a discrete solution trajectory $\{(t_i, x_i)\}_{i \in [N]}$ as input, which we obtain by integrating $\dot{x} = f(x)$ for a random initial condition.
%, after which we add noise and randomly drop some observations.

%We describe our data generation procedure in \cref{sec:generation}, model choices and innovations in \cref{sec:method}, evaluation methods in \cref{sec:experiments} and finally benchmarks and results in \cref{sec:results}.
%Our code, models and benchmark dataset are available publicly at
%\texttt{anonymized}.
% ~\url{https://github.com/sdascoli/odeformer}. We also released a pip package entitled \texttt{odeformer} for easy setup and usage.


\section{Related Work}\label{sec:related_work}

%%%%
% UPDATED SOME PARAGRAPHS IN THIS SUBSECTION DIRECTLY. HOPE THAT'S OK
\xhdr{Modeling dynamical systems.}
We briefly mention some relevant cornerstones from the long history of modeling dynamical systems from data, each of which has inspired a large body of follow-up work.
%it is limited to ground truth functions that are a linear combination of these basis functions and only the coefficients have to be inferred.
Neural ODEs (NODE)~\citep{chen2018neural} parameterize the ODE $f$ by a neural network and train it by backpropagating through ODE solvers (either directly or via adjoint sensitivity methods).
NODEs require no domain knowledge but only represent the dynamics as a generally overparameterized black-box model void of interpretability.
Assuming 
%a different kind of 
prior knowledge about the observed data, physics-informed neural networks~\citep{raissi2019physics,karniadakis2021physics} aim to model dynamical systems using neural networks regularized to satisfy a set of physical constraints.
This approach was recently extended to uncover unknown terms in differential equations~\citep{podina2023universal}. 
In this work, we aim to infer interpretable dynamical equations when no domain knowledge is available.
%%%%
%Assuming prior knowledge about the observed data, physics-informed neural networks~\citep{raissi2019physics} aim to model dynamical systems using neural networks regularized to satisfy a set of physical constraints.
%Recently, this approach has been extended to uncover unknown terms in differential equations~\citep{podina2023universal}.
%Finally, Neural ODEs (NODE)~\citep{chen2018neural} parameterize the ODEs $f$ by a neural network and train it by backpropagating through ODE solvers (either directly or via the adjoint sensitivity method).
%NODEs require no domain knowledge, but only represent the dynamics as a generally overparameterized black-box model void of interpretability.
%In this work, we aim to infer interpretable dynamical equations in the setting where no domain knowledge is available.
%%%%


% where the time component corresponds to the depth of the network. In this case, no domain knowledge is assumed, but the resulting model of the dynamical system is generally an overparameterized function void of interpretability.

\xhdr{Approaches to symbolic regression.}
% NEW TEXT
Symbolic regression aims to find a concise mathematical function that accurately models the data. While it is possible to generate complex analytical expressions that fit the observations, an unnecessarily lengthy function is often impractical. Symbolic regression seeks a balance between fidelity to the data and simplicity of form.
% Symbolic regression aims to provide a mathematical function in symbolic form that fits the observations while remaining parsimonious -- an analytical expression that spans pages may still be useless.
Therefore, predictions are typically also evaluated in terms of some ``complexity'' metric.
Because the symbolic output makes it difficult to formulate differentiable losses, SR has traditionally benefitted comparably little from advances in autodifferentiation and gradient-based optimization frameworks.
The dominant approach has thus been based on evolutionary algorithms such as genetic programming (GP)
\citep{la2016epsilon,la2018learning,kommenda2020genetic,virgolin2021improving,tohme2022gsr,cranmer2023interpretable}, optionally guided by neural networks~\citep{mundhenk2021symbolic,udrescu2020ai,costa2021fast} and recently also employing reinforcement learning \citep{petersen2020deep} -- see~\citep{la2021contemporary,makke2022interpretable} for reviews.
Most of these approaches require a separate optimization for each new observed system, severely limiting scalability.

% OLD TEXT
% Symbolic regression consists in search for a mathematical function which fits the observations as well as possible, and stands as an ideal compromise between powerful but uninterpretable models such as Neural ODEs and interpretable but simplistic approaches such as SINDy. Yet, SR is still today a rather unexplored paradigm in the machine learning literature. Indeed, this search cannot directly be framed as a differentiable problem, and the dominant approach for SR is that of genetic programming (GP) \citep{koza,schmidt2009distilling,todorovski1997declarative,bridewell2008inductive,schmidt2010age,mcconaghy2011ffx,arnaldo2014multiple,la2016epsilon,la2018learning,kommenda2020genetic,virgolin2017scalable,virgolin2019linear,burlacu2020operon,simidjievski2020equation,virgolin2021improving,de2021interaction,tohme2022gsr,mundhenk2021symbolic} (see~\citep{la2021contemporary,makke2022interpretable} for recent reviews). However, SR has also seen growing interest from the deep learning community, motivated by the fact that neural networks are extremely powerful at identifying qualitative patterns. Neural networks have been used to aid genetic programming algorithms, e.g., by simplifying the original dataset~\citep{udrescu2020ai} or proposing a good starting distribution over mathematical expressions\citep{petersen2019deep}. Conversely, genetic algorithms have been used to interpret the latent space of neural networks~\citep{Cranmer2020DiscoveringSM}. 

\xhdr{Transformers for symbolic regression.}
With the advent of transformer models~\citep{vaswani2017attention}, efficient learning of sequence-to-sequence tasks for a broad variety of modalities became feasible.
Paired with large-scale pre-training on synthetic data, transformers have been used for symbolic tasks such as integration~\citep{lample2019deep}, formal logic~\citep{hahn2020teaching}, and theorem proving~\citep{polu2020generative}.
Few recent works applied them to functional SR~\citep{biggio2021neural,valipour2021symbolicgpt,kamienny2022end,vastl2022symformer} obtaining comparable results to GP methods, with a key advantage: after one-time pre-training, inference is often orders of magnitude faster since no training is needed for previously unseen systems.
% Indeed, while the latter need to be ran from scratch on each new set of observations, language models are pre-trained over vast synthetic datasets from which they can leverage past experience.
\citet{landajuela2022unified} recently proposed a hybrid system combining and leveraging the advantages of most previous approaches for state of the art performance on functional SR tasks.

\xhdr{Symbolic regression for dynamical systems.}
In principle, dynamical SR, inferring $f$ from $(t, x(t))$, can be framed as functional SR for $(x(t), \dot{x}(t))$ pairs.
However, when transitioning from functional to dynamical symbolic regression, a key challenge is the absence of regression targets $\dot{x}(t)$ since temporal derivatives are usually not observed directly.
A common remedy is to use numerical approximations of the missing derivatives as surrogate targets instead. This approach has been employed in the GP community \citep{gaucel2014learning,la2016inference} and is also key to the widely used SINDy~\citep{sindy} algorithm which performs sparse linear regression on a manually pre-defined set of basis functions. While SINDy is computationally efficient, its modeling capacity is limited to linear combinations of its basis functions. 
% All existing methods mentioned so far focus on functional SR.
Like in functional SR, neural networks have also been combined with GP for dynamical SR \citep{atkinson2019data}, and the divide-and-conquer strategy by \citet{udrescu2020ai} has also been extended to inferring dynamical systems \citep{weilbach2021inferring}.
Finally, \citet{omejc2023probabilistic} recently introduced ProGED, which performs dynamical SR via random search of candidate equations, constrained by probabilistic
context-free grammars (PCFGs). This approach does not require numerical approximations to temporal derivatives, however, the parameters of the PCFGs need to be carefully tailored to each problem, which assumes prior knowledge about the ground truth.
In the realm of transformers,
\citet{d2022deep} infer one-dimensional recurrence relations in sequences of numbers, which as discrete maps are closely related to differential equations.
Most related to our work, \citet{becker2023predicting} explore a transformer-based approach to dynamical SR for ODEs.
However, their method is limited to univariate ODEs.
Such systems exhibit extremely limited behavior, where solution trajectories can only either monotonically diverge or monotonically approach a fixed value -- not even inflections let alone oscillations are possible \citep{strogatz:2000}.
In this work, we tackle the important yet unsolved task of efficiently discovering arbitrary non-linear ODE systems in symbolic form directly from data in multiple dimensions, without assuming prior knowledge of the ground truth.

\xhdr{Theoretical identifiability.}
Traditionally, the identifiability of ODEs from data has been studied in a case-by-case analysis for pre-defined parametric functions  \citep{aastrom1971system,miao2011identifiability,villaverde2016structural,hamelin2020observability}.
Recent work made progress on identifiability within function classes such as linear (in parameters) autonomous ODE systems \citep{stanhope2014identifiability,duan2020identification,qiu2022identifiability} or, in the scalar case, even non-parametric classes such as analytic, algebraic, continuous, or smooth functions \citep{scholl2023uniqueness}.
As it stands, it is difficult to gain practical insights from these results for our setting as they do not conclude whether non-linear ODEs can practically be uniquely inferred from data -- see \cref{app:identifiability} for details.

% OLD TEXT
% Our task is to infer functions $f:\mathbb R^D \to \mathbb R^D$ in differential systems of the form 
% \[ \dot x = f(x,t), \quad x\in \mathbb R^D.\] To do so, we will pre-train large language models on a vast dataset of synthetic examples, where for each example the input is a trajectory $\{(t_i, x_i)\}_{i\in[[1,N]]}$ and the target is the function $f$. Examples are generated by first sampling a random function $f$, then the input trajectories, as explained in what follows. Our general method is summarized in \cref{fig:sketch}. 

\begin{figure*}
    \centering
    % \begin{subfigure}[b]{.28\linewidth}
    % \centering
    %         \Tree
    %         [.$\mathrm{+}$ [.$\mathrm{\times}$ [.$1.3$ ][.$x_1$ ]][.$\mathrm{\times}$ [.$-2.5$ ][.$\mathrm{cos}$ [.$x_2$ ]]]]
    %         %\end{qtree}
    % \caption{The tree above represents the function $1.3x_1-2.5\cos (x_2)$}%, and is tokenized as $\texttt{[sub mul + 1300 e-3 x1 mul - 2500 e-3 cos x0]}$}
    % \label{fig:treesampling}
    % \end{subfigure} 
    % \hfill
    % \begin{subfigure}[b]{\linewidth}
    \vspace{-7mm}
    \includegraphics[width=\columnwidth]{figs/transformer.pdf}
    % \end{subfigure} 
    \vspace{-4mm}
    \caption{\textbf{Sketch of our method to train \odeformer{}}. We generate random ODE systems, integrate a solution trajectory on a grid of $N$ points $x\in \R^{\din}$, and train \odeformer{} to directly output the ODE system in symbolic form, supervising the predicted expression via cross-entropy loss.}\label{fig:sketch}
    \vspace{-5mm}
\end{figure*}

\section{Data Generation}\label{sec:generation}
Our method builds on pretraining on a large dataset of ODEs which is assembled as follows.

%\subsection{Generating and representing functions in symbolic form}\label{sec:func-generation}
\xhdr{Generating ODEs.}
For a $\din$-dimensional ODE $f$, we independently sample the $\din$ component functions $f_1, \ldots, f_{\din}$ 
%of the function $f$ 
as random unary-binary trees following the method of~\citep{lample2019deep}, where internal nodes represent mathematical operators and leaves represent constants or variables.
In our specific procedure, we first sample the system dimension $\din$ uniformly from $[\din_{\max}]$ for a fixed $\din_{\max} \in \mathbb{N}$ and then perform the following steps for each component function:
%\begin{enumerate}[leftmargin=*,noitemsep,topsep=-1mm]
%    \item Sample the number of binary operators $b$ uniformly from $[b_{\max}]$ for a fixed $b_{\max} \in \mathbb{N}$.
%    \item Sample $b$ times from the binary operators $\{+,\times\}$ with probabilities $P(+) = \tfrac{3}{4}$ and $P(\times) = \tfrac{1}{4}$.\footnote{Subtractions and divisions are included via multiplication with negative numbers and the unary operator $x \mapsto x^{-1}$ respectively. It has been argued that divisions appear less frequently than additions and multiplications in ``typical'' expressions~\citep{guimera2020bayesian}.}
%    \item Construct a binary tree with those $b$ nodes, adapting the procedure of~\citet{lample2019deep}. 
%    \item For each leaf in the tree, sample one of the variables $x_i$ for $i \in [\din]$.
%    \item Sample the number of unary operators $u$ uniformly from $[u_{\max}]$ for a fixed $u_{\max} \in \mathbb{N}$.
    %\item Sample $u$ times from the unary operators $\{x\mapsto \sin(x), x\mapsto x^{-1}, x\mapsto x^2\}$, and insert them above any node whose subtree has a depth smaller than 6.\footnote{This condition aims to avoid deeply nested -- and thus uninterpretable -- expressions, which often occur in genetic programming-based SR.}
%    \item Sample $u$ unary operators (uniformly with replacement) from $\{x\mapsto \sin(x), x\mapsto x^{-1}, x\mapsto x^2\}$, and insert them directly above any node whose subtree has a depth smaller than 6.\footnote{This aims at avoiding deeply nested uninterpretable expressions, which often occur in GP-based SR.}
%    \item The constants in the equation are samples from a log-uniform distribution on $[c_{\min}, c_{\max}]$. To achieve full generality, we ensure that each term is multiplied by a prefactor, and that the argument $x$ of each unary function is rescaled by an affine transformation $x\to a\cdot x + b$ (with $a, b$ sampled from the same log-uniform distribution).
%\end{enumerate}

\begin{enumerate}[leftmargin=*,noitemsep,topsep=-1mm]
    \item Sample the number of binary operators $b$ uniformly from $[b_{\max}]$ for a fixed $b_{\max} \in \mathbb{N}$.

\item Sample a binary tree with $b$ non-leaf nodes, following the procedure of ~\citet{lample2019deep}. 

\item Decorate each non-leaf node with a binary operator sampled from 
%$\{+,\times\}$ with probabilities 
$P(+) = \nicefrac{3}{4}$ and $P(\times) = \nicefrac{1}{4}$.\footnote{Subtractions and divisions are included via multiplication with negative numbers and the unary operator $x \mapsto x^{-1}$ respectively. It has been argued that divisions appear less frequently than additions and multiplications in ``typical'' expressions~\citep{guimera2020bayesian}.}%\tfrac{3}{4}$ and $P(\times) = \tfrac{1}{4}$.\footnote{Subtractions and divisions are included via multiplication with negative numbers and the unary operator $x \mapsto x^{-1}$ respectively. It has been argued that divisions appear less frequently than additions and multiplications in ``typical'' expressions~\citep{guimera2020bayesian}.}

\item For each leaf in the tree, sample one of the variables $x_i$ for $i \in [\din]$.

\item Sample the number of unary operators $u$ uniformly from $[u_{\max}]$ for a fixed $u_{\max} \in \mathbb{N}$.

\item Iteratively with $u$ repetitions, select a node whose subtree has a depth smaller than 6\footnote{This aims at avoiding deeply nested uninterpretable expressions, which often occur in GP-based SR.} and insert a new node directly above. Populate the new node with a unary operator that is sampled uniformly at random from $\{x\mapsto \sin(x), x\mapsto x^{-1}, x\mapsto x^2\}$.

\item Convert the tree into a mathematical expression via preorder traversal \citep{lample2019deep}.

\item Finally, prepend a coefficient to each term and wrap the argument of any unary operator in an affine transformation $x\to a\cdot x + b$. Coefficients and constants of affine transformations are sampled independently from a log-uniform distribution on $[c_{\min}, c_{\max}]$.

%\item The constants in the equation are samples from a log-uniform distribution on $[c_{\min}, c_{\max}]$. To achieve full generality, we ensure that each term is multiplied by a prefactor, and that the argument $x$ of each unary function is rescaled by an affine transformation $x\to a\cdot x + b$ (with $a, b$ sampled from the same log-uniform distribution).
\end{enumerate}


% \footnote{ a larger range leads to negligible or exploding terms.}
%We provide our reasoning behind these numbers and sampling choices in \missing{refer to appendix}.
Due to random continuous constants (and initial conditions), we almost surely never sample a function twice.
In our experiments, we use $\din_{\max}=6$, $b_{\max} = 5$, $u_{\max} = 3$, $(c_{\min}, c_{\max}) = (0.05, 20)$.


%\subsection{Integrating ODEs to obtain solution trajectories}

\xhdr{Integrating ODEs.}
Once the function $f$ is generated, we sample an initial condition $x_0 \sim \mathcal{N}(0, \gamma \mathbb{I}_D)$ for a fixed $\gamma \in \R_{> 0}$ and $\mathbb{I}_D$ the identity matrix, and integrate the ODE from $t=1$ to $t=T$ using the numerical solver $\texttt{scipy.integrate.solve\_ivp}$ provided by SciPy~\citep{virtanen2020scipy} on a fixed homogeneous grid of $N$ points, where $N$ is sampled uniformly in $\{50, 51, \ldots, 200\}$.
The \texttt{solve\_ivp} function defaults to an adaptive 5th order explicit Runge Kutta method with 4th order error control \citep{dormand1980family} as well as relative and absolute tolerances of $10^{-3}$ and $10^{-6}$ respectively.
When integration fails, i.e., when the solver throws an error, returns unsuccessfully, or takes longer than one second, we simply discard the current example.
\Cref{sec:method} explains in detail that we can fix $T$ and $\gamma$ during training without loss of generality, as we can rescale observations at inference time.
Hence, we fix $\gamma = 1$ and $T = 10$ during training.

% OLD
% In order for the model to be insensitive to the scale and the time interval considered at inference, one could imagine sampling different values for the parameters $\sigma$ and $T$ at each new example during training.
% However, as explained in \cref{sec:inference}, this is not necessary: one can simply rescale the trajectories at inference, allowing to always use $\sigma=1$ and $T=10$ during training.

\xhdr{Filtering data.}
Under the distribution over functions $f$ defined implicitly by our generator, a substantial fraction of sampled ODEs (and initial conditions) leads to solutions where at least one component diverges over time.
Continued divergence over long time spans is typically deemed ``unphysical''.
Among the trajectories that remain finite, we observe that again a substantial fraction swiftly converges towards a fixed point.
Although these solutions may be realistic, their dominance hampers diversity in our dataset. Also, stable constant observations over long times spans are arguably rarely of interest.
Hence, we use the following heuristics to increase diversity of the generated ODEs.
\begin{itemize}[leftmargin=0.5cm,nosep]
    \item If any variable of the solution trajectory exceeds a fixed threshold ($10^2$ in our experiments), we discard the example.
    This amounts to filtering out divergent systems.
    \item If the oscillation of all component functions over the last quarter of the integration range is below a certain threshold ($10^{-3}$ in our experiments), we discard the example with a probability of 90\%.\footnote{The oscillation of a function $h: [a, b] \to \R$ is given by $\sup_{x \in [a,b]} h(x) - \inf_{x \in [a,b]} f(x)$.}
    This filters out a majority of rapidly converging systems.
\end{itemize}

\xhdr{Corrupting data.}
We apply two forms of corruption to the clean solution trajectories:
%We apply two forms of corruption to the clean, homogeneously integrated solution trajectories during training.
\begin{itemize}[leftmargin=0.5cm,nosep]
    \item \emph{Noise:} We sample a noise level $\sigma$ uniformly in $[0,0.1]$ and corrupt each observation of each component of the trajectory independently multiplicatively with Gaussian noise: $x_j(t_i) \to (1 + \xi) x_j(t_i)$ for $j \in [D], i \in [N]$ and $\xi \sim \mathcal{N}(0, \sigma)$.
    This noise model has been used and argued for in previous works \citep{d2022deep,becker2023predicting}.
    \item \emph{Subsampling:}  For each trajectory, we sample a subsampling ratio $\rho$ uniformly in $[0,0.5]$ and drop a fraction $\rho$ of the points along the trajectory uniformly at random.
    Since the equally spaced original trajectories contained between 50 and 200 points, after subsampling inputs can vary in length between 25 and 200.
\end{itemize}

%\subsection{Tokenizing inputs (solutions) and targets (symbolic functions)}



\section{Model, Training, and Inference}\label{sec:method}


%\subsection{Model architecture and training}

\odeformer{} is an encoder-decoder transformer ~\citep{vaswani2017attention} for end-to-end dynamical SR, illustrated in \cref{fig:sketch}. The model comprises 16 attention heads and an embedding dimension of 512, leading to a total parameter count of 86M. As observed by~\cite{charton2021linear}, we find that optimal performance is achieved in an asymmetric architecture, using 4 layers in the encoder and 16 in the decoder. Since the time component is explicitly included in the inputs, we remove positional embeddings from the encoder. Model optimization follows established procedures, with details given in \cref{app:training_details}.

\xhdr{Tokenizing numbers.}
%Following~\citet{charton2021linear}, we represent numbers in base $10$ floating-point notation, round them to four significant digits, and encode them as sequences of 3 tokens: their sign, mantissa (between \texttt{0} and \texttt{9999}), and exponent (from \texttt{E-100} to \texttt{E100}). 
Since numeric input trajectories as well as symbolic target sequences may contain floating point values, we need an efficient encoding scheme that allows the infinite number of floats to be sufficiently well conserved by a fixed-size vocabulary.
Following \citet{charton2021linear}, each number is rounded to four significant digits and disassembled into three components: sign, mantissa and exponent, each of which is represented by its own token. This tokenization scheme condenses the vocabulary size to represent floating point values to just 10203 tokens (\texttt{+}, \texttt{-}, \texttt{0}, ..., \texttt{9999}, \texttt{E-100}, ..., \texttt{E100})  and works well in practice despite the inherent loss of precision.
We also experimented with three alternative representations:
(i) two-token encoding, where the sign and mantissa are merged together,
(ii) one-token encoding where sign, mantissa and exponent are all merged together,
(iii) a two-hot encoding inspired by \citet{schrittwieser2020mastering} and used by \citet{becker2023predicting}, which interpolates linearly between fixed, pre-set values to represent continuous values.
These representations have the advantage of decreasing sequence length, and (iii) has the added benefit of increased numerical precision for the inputs.
Since all three alternatives led to worse overall performance, we used the three token representation (sign, mantissa, exponent).% for \odeformer{}.
% , indicating that explicitly stating the sign and scale of a number as two extra numbers provides a useful inductive bias.

\textbf{Embedding numerical trajectories.}
The above tokenization scheme scales the length of numerical input sequences by a factor of three. 
Points $(t_i,x_i) \in \R^{\din+1}$ of the trajectory of a $\din$ dimensional ODE system are hence mapped to a token sequence of dimension $\R^{(\din+1) \times 3}$. 
We feed the token sequence of each dimension separately to an embedding layer and concatenate the result to obtain a representation in $\R^{((\din+1) \times 3) \times \demb}$. 
Before handing this representation to the encoder it is reduced such that each original input point corresponds to a single embedding vector ~\citep{kamienny2022end}, effectively scaling the input sequence back to its original length. 
For this, potentially vacant input dimensions are padded up to $D_{\max}$ before the resulting $3 \times (D_{\max} + 1) \times \demb$-dimensional vector is processed by a 2-layer fully-connected feed-forward network (FFN) with Sigmoid-weighted linear unit (SiLU) activations~\citep{elfwing2018sigmoid}, which projects down to dimension $\demb$. This embedding process allows a single trained model to flexibly handle input trajectories of variable lengths as well as ODE systems of different dimensionalities.

%\odeformer{} is designed to take $N$ input points $(t_i,x_i) \in \R^{\din+1}$, where each input point is expressed by $3(\din+1)$ tokens of dimension $\demb$. To limit the length of input sequences, we use an embedding module to map each input point to a single embedding, following~\cite{kamienny2022end}. This embedder pads the vacant input dimensions up to $D_{\max}$, and then feeds the $3(\din_{\max} + 1) \demb$-dimensional vector into a 2-layer fully-connected feed-forward network (FFN) with Sigmoid-weighted linear unit (SiLU) activations~\citep{elfwing2018sigmoid}, which projects down to dimension $\demb$.

\xhdr{Encoding symbolic functions.}
%To depict mathematical functions in sequence form, we enumerate the trees using prefix order, also known as direct Polish notation, following~\cite{lample2019deep}. 
To encode mathematical expressions, the vocabulary of the decoder includes specific tokens for all operators and variables, in addition to the tokens used to represent floating point values. Importantly, the decoder is trained on expressions in prefix notations to relieve the model from predicting parentheses ~\citep{lample2019deep}.
%We use specific tokens to denote operators, integers, and variables. The method of encoding constants is the same as explained previously. 
With these choices, the target sequence for an exemplary ODE $f(x)=\cos(2.4242 x)$ corresponds to following sequence of six tokens $\texttt{[cos\ mul\ +\ 2424\ E-3\ x]}$.
%As an illustration, 
%the ODE $f(x)=\cos(2.4242 x)$ converts into a sequence of six tokens, namely $\texttt{[cos\ mul\ +\ 2424\ E-3\ x]}$. 
%It is worth noting that the decoder's vocabulary comprises a blend of numeric and symbolic tokens (operators and variables), while the encoder's vocabulary has only numeric tokens. For complete generality, the numeric token embeddings are \emph{not} mutually shared between the encoder and decoder.
For $\din$-dimensional systems, we simply concatenate the encodings of the $\din$ component functions, separated by a special token ``$\texttt{|}$''.
With this simple method, the sequence length scales linearly with the dimensionality of the system, i.e., the number of variables.
While this is unproblematic for small dimensions such as $\din \le \din_{\max} = 6$, it may impair the scalability of our approach.\footnote{A possible alternative would be to treat the decoding of each component function as a separate problem, adding a specifier to the $\texttt{BOS}$ (beginning of sequence) token to identify which component is to be decoded.}
As the encoder is only concerned with numeric input trajectories, its vocabulary only includes tokens for numbers.

%\textbf{Transformer.} 
%We use a sequence-to-sequence transformer~\citep{vaswani2017attention} using 16 attention heads and an embedding dimension of 512, leading to a total parameter count of 86M. As observed by~\cite{charton2021linear}, we find that optimal performance is achieved in an asymmetric architecture, using four layers in the encoder and sixteen in the decoder. Since the time component is explicitly included in the inputs, we remove positional embeddings from the encoder.

%\textbf{Training.}  
%We optimize a cross-entropy loss with the Adam optimizer (with default parameters suggested by~\cite{kingma2014adam}), with a learning rate warming up from $10^{-7}$ to $2\times 10^{-4}$ across the initial 10,000 steps, by decaying via the cosine schedule for the next 300,000 steps. The annealing cycle then restarts with a damping factor of 3/2 as per~\cite{kingma2014adam}, resulting in approximately 800,000 optimization steps. We do not use any regularization such as weight decay or dropout. To efficiently manage the greatly varying input sequence lengths, we group examples of similar lengths in batches, with the constraint that each batch contains 10,000 tokens. Our model is trained on a set of about 50M examples pre-generated with 80 CPU cores. When run on a single NVIDIA A100 GPU with 80GB memory and 8 CPU cores, \odeformer{}’s training process takes roughly three days.


%\subsection{Inference}\label{sec:inference}

\xhdr{Rescaling.}
During training, the model only observes initial conditions from a standard normal distribution, and the integration range is fixed to $[1,10]$.
% At inference, the scale of the initial conditions and the time range can be different.
To accommodate for different scales of initial conditions and time ranges during inference, we apply the affine transformations $t \to \tilde{t} = a t + b$ to rescale the observed time range to $[1,10]$ and $x_i(t) \to \tilde{x}_i(t) = \tfrac{x_i(t)}{x_i(t_0)}$ to rescale initial values to unity. 
The prediction $\tilde{f}$ that \odeformer{} provides on inputs $(\tilde{t}, \tilde{x})$ are then transformed as $f_i = \tfrac{dx_i}{dt} = \tfrac{1}{ax_i(t_0)}\tfrac{d\tilde{x}_i}{d\tilde{t}} = \tfrac{1}{a x_i(t_0)}\tilde{f_i}$ to recover original units.

\xhdr{Decoding strategy.}
At inference, we use beam sampling \citep{van2008beam} to decode candidate equations, and select the candidate with highest reconstruction $R^2$ score.\footnote{Beam search tends to produce candidates which all have the same skeleton, and only differ by small variations of the constants, leading to a lack of diversity. Beam sampling ensures that randomness is added at each step of decoding leading to a more diverse set of candidate expressions.}
The beam temperature is an important parameter to control diversity -- as the beam size increases, it typically becomes useful to also increase the temperature to maintain diversity.
Unless stated otherwise, we perform our experiments with a beam size of 50 and a temperature of 0.1.

\xhdr{Optional parameter optimization.}
Most SR methods break the task into two subroutines (possibly alternating between the two): predicting the optimal ``skeleton'', i.e., equation structure, and fitting the numerical values of the constants.
Just like~\citet{kamienny2022end}, our model is end-to-end, in the sense that it handles both subroutines simultaneously.
However, we also experimented with adding an extra parameter optimization step, as performed in methods such as ProGED~\citep{omejc2023probabilistic}. We describe the details of the parameter optimization procedure in \cref{app:optional_parameter_optimization} and denote this method as ``\odeformer{} (opt)''.
%While we observe marginal gains in fitting power, this method does not improve generalization and can lead to overfitting when the data is noisy -- see the results in \cref{sec:results}, where the model with additional constant optimization is denoted as ``\odeformer{} (opt)''.

\section{Evaluation}\label{sec:experiments}

\xhdr{Symbolic vs numerical evaluation.}
When evaluating SR methods, the desired metric is whether the inferred ODE $\hat{f}$ perfectly agrees symbolically with the ground truth expression $f$.
However, such an evaluation is problematic primarily because
(i) the ambiguity in representing mathematical expressions and non-determinism of ``\texttt{simplify}'' operations in modern computer algebra systems render comparisons on the symbolic level difficult, and
(ii) expressions may differ symbolically, while evaluating to essentially the same outputs on all possible inputs (e.g., in the presence of a negligible extra term).
%(iv) Even if we could reliably compare symbolic expressions, it remains hard to define a continuous metric beyond a binary equal/unequal relation. 
Hence, comparing expressions numerically on a relevant range is more reliable and meaningful.
Even modern computer algebra systems include numerical evaluations in equality checks, which still require choosing a range on which to compare expressions \citep{meurer2017sympy}.

\xhdr{Evaluation types.}
For dynamical SR there is a spectrum of reasonable comparisons.
We could simply be interested in finding \emph{some} ODE $\hat{f}$, whose solution approximates the observed trajectory $x(t)$ on the observed time interval, even if $\hat{f}$ still differs from $f$ on (parts of) their domain.
A more ambitious goal closer to full identification is to find a 
%$\hat{f}$ such that the solution trajectory correctly extrapolates beyond the observed time span for the same initial condition, or a 
$\hat{f}$ that also approximates the correct trajectories for unobserved initial conditions.
This evaluation, which in our view is most meaningful to assess dynamical SR, is often absent in the literature, e.g., from \citet{omejc2023probabilistic}.
%who instead use manual symbolic heuristics.
If an inferred $\hat{f}$ yields correct solutions for all initial values and time spans, we would consider it as perfect identification of $f$.
Accordingly, we evaluate the following aspects of performance in our experiments.
% \xhdr{Fitting error and generalization error.}
% We assess the quality of predictions numerically, by integrating the ODE and checking how close the predicted trajectory is to the true trajectory. We consider two settings for the numerical evaluation, depending on the choice of initial conditions:
\begin{itemize}[leftmargin=0.5cm,nosep]
    \item \emph{Reconstruction:} we compare the (noiseless, dense) ground truth trajectory with the trajectory obtained by integrating the predicted ODE from the same initial condition and on the same interval $[1,T]$ as the ground truth.
%    \item \textbf{Forecasting:} we compare the (noiseless, dense) ground truth trajectory beyond the observed time span with the one we get from integrating the predicted ODE from the same initial condition beyond $T$.
    %\missing{How long is the forecasting?}
    % more importantly, we want to check how close the prediction is to the ground truth at the symbolic level. In the dynamical setup considered here, a good proxy for generalization can be obtained by considering a different initial condition, and comparing the trajectories integrated from the ground truth and the predicted ODEs.
    \item \emph{Generalization:} we integrate both the ground truth and the inferred ODE for a new, different initial condition over the same interval $[1,T]$ and compare the obtained trajectories.
\end{itemize}

\xhdr{Metrics.}
%Even having fixed the types of evaluation, the exact quantitative comparison metrics pose a non-trivial problem in SR.
We consider the following performance metrics.
\begin{itemize}[leftmargin=0.5cm,nosep]
    \item \emph{Accuracy:} A classical performance metric for regression tasks is the coefficient of determination, defined as $R^2 = 1-\frac{\sum_i\left(y_i-\hat{y}_i\right)^2}{\sum_i\left(y_i-\bar{y}\right)^2} \in (-\infty, 1]$. Since $R^2$ is unbounded from below, average $R^2$-scores across multiple predictions may be severely biased by even a single particularly poor outlier. We therefore instead report the percentage of predictions for which the $R^2$ exceeds a threshold of 0.9 in the main text and show the distribution of scores in \cref{app:results}.
    
    %\item \emph{$R^2$ score:} this is the coefficient of determination classically used for regression tasks, defined as $R^2 = 1-\frac{\sum_i\left(y_i-\hat{y}_i\right)^2}{\sum_i\left(y_i-\bar{y}\right)^2} \in (-\infty, 1]$.
    %Since $R^2$ is unbounded from below, aggregating $R^2$-scores over multiple examples via averaging may suffer from a few unusually bad outliers.
    %Therefore, we mostly report median $R^2$-scores over the different datasets.
    % a single bad prediction can lead the average $R^2$ to explode -- to avoid this, as in ~\citep{biggio2021neural}, we in fact compute $\max(0, R^2)$, under the rationale that the trivial predictor $\hat y = \bar y$ achieves $R^2=0$.
    %\item \emph{Accuracy:} following~\cite{la2021contemporary}, we define accuracy to be 1, if the $R^2$ score exceeds a threshold, and 0 otherwise. Given the difficulty of dynamical SR, we set the threshold to 0.9. %following~\citet{biggio2021neural}, we use $\texttt{np.allclose}$ with absolute and relative tolerances of $10^{-3}$ and $0.05$ respectively as a binary measure of whether trajectories agree.
    \item \emph{Complexity:} we define the complexity of a symbolic expression to be the total number of operators, variables and constants. We acknowledge that this is a crude measure, for example, it would assign a lower complexity to $\exp(\tan(x))$ (complexity=3) than to $1+2x$ (complexity=5).
    Yet, there is no agreed-upon meaning of the term ``complexity'' for a symbolic expression in this context so that
    simply counting ``constituents'' is common in the literature, see e.g. the discussion in the benchmark by \citet{la2021contemporary}.
    \item \emph{Inference time:} time to produce a prediction. %Note that all methods except ours require hyperparameter tuning: we do \emph{not} take this into account in the inference time. 
\end{itemize}

\begin{figure}[htb]
    \centering
    % \vspace{-9mm}
    \includegraphics[width=\linewidth]{figs/acc_vs_info.pdf}
    \caption{\textbf{Ablation study on synthetic data.} We vary four parameters governing the difficulty of an example (from left to right): the dimension of the system, the total number of unary and binary operators, and the number of points in the trajectory. In each panel, we average the results over a dataset of 10,000 examples. In all cases, we use a beam size of 50.}\label{fig:synthetic}
    \vspace{-6mm}
\end{figure}

\xhdr{Corruptions.}
For all datasets, we also compare models on their robustness to two types of corruption: (i) we add noise to the observations via $x_j(t_i) \to (1 + \xi) x_j(t_i)$ for $j \in [D], i \in [N]$ and $\xi \sim \mathcal{N}(0, \sigma)$; (ii) we drop a fraction $\rho$ of the observations along the trajectory uniformly at random.
We report results for various noise levels $\sigma$ and subsampling fractions $\rho$.
% \begin{itemize}[leftmargin=]
    % \item \textbf{Noise:} we corrupt the trajectories with a multiplicative noise of variance $\sigma$: $x_i(t) \to (1+\xi(t))x_i(t), \xi(t)\sim\mathcal N(0,\sigma)$.
    % \item \textbf{Subsampling:} then randomly remove a fraction $\rho$ of the points along the trajectory. 
% \end{itemize}



% For evaluations on corrupted (noisy and irregularly sampled) data, the corrupted trajectory is used for candidate selection, but final performance is always reported on clean (noiseless, dense) trajectories.

\xhdr{Results on synthetic data.}
We first assess how the performance of \odeformer{} is affected by the dimensionality of the ODE system, the number of unary and binary operators, and the number of points in the trajectory.
The ablation results on 10,000 synthetic examples with a beam size of 50 are shown in \cref{fig:synthetic} -- we asses the effect of the beam size in \cref{app:beamsize}. We make three observations:
\begin{itemize}[noitemsep, leftmargin=0.5cm,topsep=-1mm]
    \item Performance degrades with the first three parameters as expected, but \odeformer{} is surprisingly insensitive to the number of points in the trajectory.
    \item Generalization accuracy is substantially lower than reconstruction accuracy as expected, but at least for low-dimensional systems we achieve non-trivial generalization (e.g., 60\% generalization accuracy vs 85\% reconstruction accuracy for 1D).
    \item \odeformer{} copes well with subsampling, but suffers more from noisy trajectories. However, the effect on generalization is smaller than that on reconstruction.
\end{itemize}
% This hints at the fact that our model mainly relies on high-level features, which are preserved even in the low-data regime, rather than on details.

% \xhdr{Fitting and generalization.}
% This shows that \odeformer{} is capable of 
%However, these results also emphasize that generalization to new initial conditions remains an exceedingly difficult task.
%, suggesting that it regularly correctly recovers the ground truth ODE.
% We also investigate the robustness to irregularly sampled and noisy data by adding 5\% noise ($\sigma = 0.05$) and subsampling 10\% of the data points ($\rho=0.1$).





\section{Benchmarking Dynamical Symbolic Regression Methods}\label{sec:results}

\xhdr{Strogatz benchmark.}
We first consider the ``Strogatz dataset'', included in the Penn Machine Learning Benchmark (PMLB) database \citep{la2021contemporary}.
It consists of seven ODE systems and has been used as a benchmark by various SR methods, in particular those specialized on dynamical SR \citep{omejc2023probabilistic}.
However, it has several limitations: (i) it is small (only seven unique ODEs, each integrated for 4 different initial conditions), (ii) it only contains 2-dimensional systems, (iii) it is not integrated with sufficient precision \citep{omejc2023probabilistic}, and (iv) its annotations are misleading (e.g., claiming that all systems develop chaos even though none of them does).
% and, (iv) all existing methods typically fail to recover the ground truth equations, hinting to a potential unidentifiability problem~\citep{scholl2023uniqueness}.

\xhdr{\odebench{}.}
Faced with these limitations, we introduce  \odebench{}, an extended benchmark curated from ODEs that have been used by \citet{strogatz:2000} to model real-world phenomena as well as well-known systems from Wikipedia.
We fix parameter values to obtain the behavior the models were developed for, and choose two initial conditions for each equation to evaluate generalization.
\odebench{} consists of 63 ODEs (1D: 23, 2D: 28, 3D: 10, 4D: 2), four of which exhibit chaotic behavior.
%contains all ODEs in the Strogatz dataset (with different parameters and initial conditions).
We publicly release \odebench{} with descriptions, sources of all equations, and well integrated solution trajectories -- more details are in \cref{app:odebench}.


\xhdr{Baselines.}
In our experiments, we extensively compare \odeformer{} with (strong representatives of) existing methods described in \cref{tab:baselines}.
For each baseline model, we perform a separate hyperparameter optimization for each run to ensure maximal fairness.
Apart from ProGED and SINDy, all baselines were developed for functional SR. We use them for dynamical SR as described in \cref{sec:related_work}, by computing temporal derivatives $\dot{x}_i(t)$ via finite differences with hyperparameter search on the approximation order and optional use of a Savitzky-Savgol filter for smoothing. For more details, please refer to \cref{app:baselines}. Note that our method is the only one which does not require any hyperparameter tuning or prior knowledge on the set of operators to be used.


% \xhdr{Synthetic data.}
% Given the difficulty of obtaining textbook systems of dimensions larger than 2, we also evaluate all methods on a synthetic dataset of high-order ODE systems (up to dimension 6).
% Note that this dataset is sampled from the training distribution of the \odeformer{} (in distribution but out of sample), which could give our model an unfair advantage.

%\begin{figure}[htb]

\begin{table*}[htb]
\centering
\caption{\textbf{Overview of models.} f.d.: finite differences required, ode: method developed for dynamical SR, T: transformer-based, GP: genetic programming, MC: Monte Carlo, reg: regression}
\vspace{-3mm}
\label{tab:baselines}
{\small
\begin{tabular}{cccccc}
  \toprule
    \textbf{name} & \textbf{type} & \textbf{ode} & \textbf{f.d.} & \textbf{description} & \textbf{reference} \\ \midrule
    ODEFormer & T & yes & no & seq.-to-seq. translation& ours\\
    AFP        & GP & no & yes & age-fitness Pareto optimization & \citep{schmidt2011age} \\
    FE-AFP     & GP & no & yes & AFP with co-evolved fitness estimates & \citep{schmidt2011age} \\
    EHC        & GP & no & yes & AFP with epigenetic hillclimbing  & \citep{la2016thesis} \\
    EPLEX      & GP & no & yes & epsilon-lexicase selection & \citep{la2016epsilon} \\
    %FEAT       & GP & no & yes & learned differentiable features & \citep{la2018learning} \\
    PySR       & GP & no & yes & AutoML-Zero + simulated annealing & \citep{cranmer2023interpretable} \\
    SINDy      & reg    & yes & yes & sparse linear regression & \citep{sindy} \\
    FFX        & reg    & no & yes & pathwise regularized ElasticNet regression & \citep{mcconaghy2011ffx} \\
    ProGED     & MC   & yes & no & MC on probabilistic context free grammars & \citep{omejc2023probabilistic} \\
    \bottomrule
\end{tabular}}%
\end{table*}

\def\squeeze{-6mm}
\begin{figure}[htb]
    \centering
        \vspace{-2mm}
        \hspace{2cm}
        \begin{subfigure}[b]{0.8\linewidth}
        %\begin{subfigure}[b]{0.5\linewidth}
        \includegraphics[width=\linewidth]{figs/baseline_comparison/final/baseline_comparison_legend.pdf}
    \end{subfigure}\\[2mm]
    \begin{subfigure}[b]{1\linewidth}
    \includegraphics[width=\linewidth]{figs/baseline_comparison/final/baseline_comparison_strogatz_all_subsample_ratios_interpolation_adaptive_additive_test_r2_threshold_0.9.pdf}
        %\vspace{\squeeze}
        \caption{Reconstruction on Strogatz}
    \end{subfigure}\\[2mm]
    \begin{subfigure}[b]{1\linewidth}
        \includegraphics[width=\linewidth]{figs/baseline_comparison/final/baseline_comparison_strogatz_extended_all_subsample_ratios_interpolation_adaptive_additive_test_r2_threshold_0.9.pdf}
        %\vspace{\squeeze}
        \caption{Reconstruction on \odebench{}}
    \end{subfigure}
    %\begin{subfigure}[b]{1\linewidth}
    %    \includegraphics[width=\linewidth]{figs/baseline_comparison/strogatz/final/testing/baseline_comparison_strogatz_extended_all_subsample_ratios_y0_generalization_adaptive_additive_test_r2_threshold_0.9.pdf}
    %    \vspace{\squeeze}
    %    \caption{Generalization on \odebench{}}
    %\end{subfigure}
    \vspace{-4mm}
    \caption{\textbf{Our model achieves state-of-the art performance on both benchmarks considered, while achieving higher robustness to noise and irregular sampling.} We compare \odeformer{} with and without additional parameter optimization using existing methods following the protocol described in \cref{sec:results}. We present results for two values of the subsampling parameter $\rho$ and six values of the noise parameter $\sigma$. Whiskers in box plot panels mark minimum and maximum values.}\label{fig:benchmarks}
    \vspace{-4mm}
\end{figure}

\xhdr{Reconstruction results.} %Qualitatively, \odeformer{} achieves excellent results on \odebench{} (\cref{fig:odebench-odeformer}). 
We present results on both ``Strogatz'' and \odebench{} in \cref{fig:benchmarks}. From top to bottom, we ranked methods by their average accuracy across all noise and subsampling levels.
The ranking is similar on the two benchmarks and \odeformer{} achieves the highest average score on both. 
The two leftmost panels show that \odeformer{} is only occasionally outperformed by PySR when the data is very clean -- as noise and subsampling kick in, \odeformer{} gains an increasingly large advantage over all other methods.
%Interestingly, \odeformer{} actually performs better on average when the trajectories are subsampled, arguably because of the subsampling during training: a perfectly homogeneous grid may constitute a distribution shift.
In the two rightmost panels of \cref{fig:benchmarks}, we show the distributions of complexity and inference time. \odeformer{} runs on the order of seconds, versus minutes for all other methods except SINDy, while maintaining relatively low and consistent equation complexity even at high noise levels. We show figures for all predictions in \cref{app:odebench}.

\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-0.5cm}
    \begin{minipage}{1\linewidth}
        \includegraphics[width=\linewidth]{figs/baseline_comparison/final/baseline_comparison_legend_large.pdf}
        \includegraphics[width=\linewidth]{figs/baseline_comparison/final/baseline_comparison_strogatz_extended_all_subsample_ratios_y0_generalization_adaptive_additive_test_r2_threshold.pdf}%
    \vspace{-2mm}
    \caption{\textbf{Generalization on \odebench{}.} We consider the same setting as in \cref{fig:benchmarks}.}
        \label{fig:generalization}
    \end{minipage}
    \vspace{-10mm}
%\end{figure}
\end{wrapfigure}
%In a generalization analysis on \odebench{}, we find that all models generalize poorly with accuracies only going up to 50\% versus close to 100\% for reconstruction, see \cref{fig:generalization}.
\xhdr{Generalization results.} We present generalization results on \odebench{} in \cref{fig:generalization}. Consistently across all models, accuracies drop by about half, meaning that half the correctly reconstructed ODEs do not match the ground truth symbolically. This highlights the importance of evaluating dynamical SR on different initial conditions.
Note, however, that the overall rankings of the different methods is rather consistent with the reconstruction results, and
\odeformer{} achieves the best results on average thanks to its robustness to noise and subsampling.


% \begin{figure}[htb]
%     \begin{center}
%         \hspace{2cm}
%         \begin{subfigure}[b]{0.8\linewidth}
%         \includegraphics[width=\linewidth]{figs/baseline_comparison/odebench/baseline_comparison_legend.pdf}
%     \end{subfigure}
%     \end{center}%
%     \begin{center}
%     \begin{subfigure}[b]{1\linewidth}
%         \includegraphics[width=\linewidth]{figs/baseline_comparison/odebench/baseline_comparison_strogatz_extended_all_subsample_ratios_interpolation_test_r2_median_invalid=-inf.pdf}
%     \end{subfigure}
%     \end{center}
%     \caption{\textbf{Results on \odebench{}.}}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figs/strogatz.pdf}
%     \caption{Strogatz datasets}
%     \label{fig:strogatz}
% \end{figure}
%\vspace{0.5cm}
\phantom{phantomtext to prevent linebreak in Discussion and future directions}
\section{Discussion and Future Directions}

We presented \odeformer{}, the first transformer capable of inferring multidimensional ODE systems from noisy, irregularly observed solution trajectories, as well as \odebench{}, a novel benchmark dataset for dynamical SR.
In extensive comparisons, we demonstrate that our model outperforms existing methods while allowing faster inference.
We foresee real-world applications of \odeformer{} across the sciences, for hypothesis generation of dynamical laws underlying experimental observations.
However, in the following we also highlight several limitations of the current method, opening up interesting directions for future work.

%First, there is inherent ambiguity and difficulty in crafting a prior over ``relevant'' or ``expected'' ODEs without focusing on a specific domain and specific prior knowledge. That said, \odeformer{} performs well on rather simple systems that are representative for ODEs found in textbooks without any specific tuning of the generator.

% as these are rather rare in the training distribution, and are very difficult to recognize qualitatively. For such systems, we believe that regression-based or GP-based algorithms will ultimately perform better. Nonetheless, we believe that although these kind of systems are extremely interesting from a theoretical point of view, they are rather rare in real-world scenarios, except in a few specific fields such as astronomy (with the three-body system as typical example).
% @Niki : do you agree with this ? This is kind of outside my expertise to be honest

First, we only considered first order ODEs.
% hence our \odeformer{} cannot predict a second order (or higher order) ODE from a single trajectory.
While any higher-order ODE can be written as a system of first order ODEs, this does not immediately allow \odeformer{} to make predictions based only on a solution trajectory, since we would still need to approximate time derivatives up to the order of the ODE. 
% one would have to approximate the additionally required initial conditions (for velocity, acceleration, etc.) from the
% Note that since an ODE of order $n$ can be expressed via $n$ first order ODEs, an easy trick to enable our system to predict a second order ODE would be to provide the model with a two-dimensional system build from the raw data and its derivatives.
While possible in principle via finite differencing schemes, we would suffer similar drawbacks as other methods that rely on finite differences from noisy, irregularly sampled data.
% However, these derivatives need to be numerically approximated via methods such as finite differencing, at the risk of introducing noise. One could adress this limitation by training the model on second order ODEs, but these would be more difficult to integrate during the data generation procedure.

Second, \odeformer{} only works when all variables are observed.
In real-world settings, some relevant variables may be unknown or unobservable.
For example, inferring chemical kinematics may be challenged by the difficulty in measuring the concentration of reaction intermediates~\citep{bures2023organic}.
We may circumvent this issue by randomly masking variables during training (replacing their observations by a dedicated token), to emulate unobserved variables.
While this raises questions around identifiability and robustness, we plan to explore masking in future work.
% which could open up many interesting applications in organic chemistry.
This technique could also handle higher-order ODEs by considering the derivatives as unobserved.

Third, based on the four representatives in \odebench{}, \odeformer{} (as well as all other benchmarked models) struggles with chaotic systems, which have been argued to provide good assessments for data-driven modeling and forecasting \citep{gilpin2021chaos}.
For chaotic systems, understanding properties of the attractor is often more desirable: nearby trajectories diverge exponentially, rendering identification notoriously challenging.
%Hence, chaotic systems are often studied over long time spans such that the attractor is traced out densely, employing different methodologies.
Dynamical law learning from short (transient) trajectories for chaotic systems remains an interesting direction for future work.

Lastly, all existing methods for dynamical SR, including ours, perform inference based on a single observed trajectory.
In our opinion, one of the most promising directions for future work is to enable inference from multiple solution trajectories of the same ODE.
Key benefits may include averaging out possible noise sources as well as improving identifiability, as we ``explore the domain of $f$''.
However, initial experiments with various forms of logit aggregation in \odeformer{}'s decoder during inference did not yield convincing results.
In future work, we plan to exploit a cross-attention encoder to combine the embeddings of the different trajectories to leverage the combined information, in the spirit of~\cite{liu2023mmvit}.

We conclude by emphasizing that the difficulty and potential ambiguity in dynamical law learning calls for caution during deployment.
Methods like \odeformer{} primarily serve as hypothesis generators, ultimately requiring further experimental verification, something that can be done well based on ODEs (rather than black-box models).
%-- especially in high-stakes settings such as health, or when deployed for model-based control of mission-critical systems.

